Interpretable Trade-offs Between Robot Task Accuracy and Compute Efficiency

A robot can invoke heterogeneous computation resources such as CPUs, cloud GPU servers, or even human computation for achieving a high-level goal. The problem of invoking an appropriate computation model so that it will successfully complete a task while keeping its compute and energy costs within a budget is called a model selection problem. In this paper, we present an optimal solution to the model selection problem with two compute models, the first being fast but less accurate, and the second being slow but more accurate. The main insight behind our solution is that a robot should invoke the slower compute model only when the benefits from the gain in accuracy outweigh the computational costs. We show that such cost-benefit analysis can be performed by leveraging the statistical correlation between the accuracy of fast and slow compute models. We demonstrate the broad applicability of our approach to diverse problems such as perception using neural networks and safe navigation of a simulated Mars rover.

==> reachablity.tex <==
\section{Offloading with Reachable Sets}
\label{sec:reachSets}
In this section, we extend our offloading algorithm to determine safety of a system through reachable sets, under the presence of uncertainties. Uncertainties in the system has been shown to have drastic effect on the reachable sets \textit{vis-à-vis} the safety; therefore, taking into account such uncertainties while determining the safety of the system is of paramount. Computing reachable sets, taking into account the uncertainties, is a computationally expensive problem. Recent works in reachable set computation with uncertainties, has provided statistical methods to compute sets with probabilistic guarantees --- given a desired probabilistic confidence by the user, a reachable set (accounting uncertainties) is computed. In this section, we extend our offloading algorithm to determine safety of a system in minimal amount of time, by leveraging a  fast (but less accurate) and a slow (more accurate) reachable set computation method.

Given a linear dynamical system with uncertainties, represented as $x^+=\Lambda x$, where $\Lambda$ is an $n$ dimensional uncertain dynamical matrix, we represent the reachable set of the uncertain system, at time step $t$, from initial set $\theta$, as $\texttt{RS}(\Lambda,\theta,t)$. 
%
Given an unsafe set $X_{unsafe}$, a system is called unsafe iff $\texttt{RS}(\Lambda,\theta,t) \cap X_{unsafe} \ne \emptyset$.
%
Given an $\delta > 0$ and $x\in \mathbb{R}^n$, $B_{\delta}(x) = \{~y~|~ ||y - x || \leq \epsilon\}$. 
%
For a set $S \subseteq \mathbb{R}^n$, $B_{\delta}(S) = \bigcup_{x \in S} B_{\delta}(x)$.
Intuitively, $B_{\delta}(S)$ is bloating the set $S$ by $\delta$.
%
We now introduce the models, loss and the reward, required to extend the offloading algorithm to perform safety verification using reachable sets.

\tu{Slow Model}: Given a linear uncertain system dynamics $\Lambda$, a time step $t$ and an initial set $\theta$, the \textit{Slow Model} returns a reachable set $\texttt{RS}_{slow}(\Lambda,\theta,t)$, \textit{s.t} $\mathbb{P} \big( \texttt{RS}(\Lambda,\theta,t) \subseteq  \texttt{RS}_{slow}(\Lambda,\theta,t)\big) \ge p_{slow}$, where $p_{slow} \in \mathbb{R}_{[0,1]}$. We assume the cost to compute $\texttt{RS}_{slow}(\Lambda,\theta,t)$ is $c_{slow}$.

\tu{Fast Model}: Given a linear uncertain system dynamics $\Lambda$, a time step $t$ and an initial set $\theta$, the \textit{Fast Model} returns a reachable set $\texttt{RS}_{fast}(\Lambda,\theta,t)$, \textit{s.t} $\mathbb{P} \big( \texttt{RS}(\Lambda,\theta,t) \subseteq  \texttt{RS}_{fast}(\Lambda,\theta,t)\big) \ge p_{fast}$, where $p_{fast} \in \mathbb{R}_{[0,1]}$. We assume the cost to compute $\texttt{RS}_{fast}(\Lambda,\theta,t)$ is $c_{fast}$. We further assume $p_{slow} > p_{fast}$ and $c_{slow} > c_{fast}$.

\tu{Relationship between the Fast and the Slow model}: Given an uncertain dynamics $\Lambda$ and an initial set $\theta$, we choose the value of $\epsilon$ to be such, that the following relationship between the \textit{Fast} and the \textit{Slow} model holds, for all time steps $t$:
\begin{eqnarray}
 &~&
 B_{1-\epsilon} \big(\texttt{RS}_{slow}(\Lambda,\theta,t) \big) \subseteq  \texttt{RS}_{fast}(\Lambda,\theta,t)  \\
 &\text{or,}&
 \texttt{RS}_{slow}(\Lambda,\theta,t) \subseteq B_{\frac{1}{1-\epsilon}} \big( \texttt{RS}_{fast}(\Lambda,\theta,t) \big)
\end{eqnarray}

\tu{Loss Function}: Let $\texttt{RS}_{fast}(\Lambda,\theta,t)=\Theta_{fast}$ and $\texttt{RS}_{fast}(\Lambda,\theta,t)=\Theta_{fast}$. The the loss function is given as:
\begin{equation}
\mathcal{L}(\Theta_{slow},\Theta_{fast}) 
=
\begin{cases}
0 & B_{\frac{1}{1-\epsilon}}(\Theta_{fast}) \cap X_{unsafe} = \emptyset \\
\infty & B_{\frac{1}{1-\epsilon}}(\Theta_{fast}) \cap X_{unsafe} \ne \emptyset
\end{cases}
\end{equation}

\tu{Reward Function}: The reward function is same as before, $i.e.$ equation \ref{eq:inference_reward}: 

\tu{Offloading}: Similar to previous cases (subsections \ref{subsec:linearReg} and \ref{subsec:dnn}), deriving from theorem \ref{thm:optimalOff}, we offload iff:
\begin{equation}
B_{\frac{1}{1-\epsilon}}(\Theta_{fast}) \cap X_{unsafe} \ne \emptyset
\end{equation}

\subsection{Experiments on Mars Rover}
\todo{1. uncertainties; 2. costs; 3. epsilon; 4. unsafe; 5: experimental setup --- waypoints, spline planner, mpc}

